Monitoring Constraints and Metaconstraints with Temporal Logics on Finite Traces

Runtime monitoring is one of the central tasks in the area of operational decision support for business process management. In particular, it helps process executors to check on-the-fly whether a running process instance satisfies business constraints of interest, providing an immediate feedback when deviations occur. We study runtime monitoring of properties expressed in LTL on finite traces (LTLf), and in its extension LDLf. LDLf is a powerful logic that captures all monadic second order logic on finite traces, and that is obtained by combining regular expressions with LTLf, adopting the syntax of propositional dynamic logic (PDL). Interestingly, in spite of its greater expressivity, \LDLf has exactly the same computational complexity of LTLf. We show that LDLf is able to declaratively express, in the logic itself, not only the constraints to be monitored, but also the de-facto standard RV-LTL monitors. On the one hand, this enables us to directly employ the standard characterization of LDLf based on finite-state automata to monitor constraints in a fine-grained way. On the other hand, it provides the basis for declaratively expressing sophisticated metaconstraints that predicate on the monitoring state of other constraints, and to check them by relying on standard logical services instead of ad-hoc algorithms. In addition, we devise a direct translation of LDLf formulae into nondeterministic finite-state automata, avoiding to detour to Buchi automata or alternating automata. We then report on how this approach has been effectively implemented using Java to manipulate LDLf formulae and their corresponding monitors, and the well-known ProM process mining suite as underlying operational decision support infrastructure.

==> 4-monitoring-coloredAutomata.tex <==
\subsection{Monitoring using Colored Automata}
\label{sec:colored-proof}

We now show that we can merge the four automata for monitoring the four RV truth values into a single automaton with ``colored'' states.
%%
The idea is grounded on the intuition that the four automata in the previous section ``have the same shape'', and only differ in determining which states are final. It is hence possible to build one automaton only and then mark its states with four different colors, each corresponding to the final states of a specific formula in Theorem~\ref{thm:rv-ltl}, hence each representing one among the four RV truth values.
%%
The intention of using a single automaton for runtime verification is not novel~\cite{MMW11}, but here, for the first time, we provide a formal justification of its correctness.

As a first step, we formally define the notion of \emph{shape equivalence} to capture the intuition that two automata have the same ``shape'', i.e., they have corresponding states and transitions, but possibly differ in their final states.


%\begin{definition}
%  \label{def:bijection}
  Formally, let $A_1 =
  (2^\Prop,\S^1,s^1_{0}, \varrho^1,
  S^1_{f})$ and $A_2 =
  (2^\Prop,\S^2,s^2_{0},\varrho^2,S^2_{f})$
  be two \NFA{s} defined over a set $\Prop$ of propositional symbols. We say that $A_1$ and $A_2$ are \emph{shape equivalent}, written $A_1 \biject A_2$, if there exists
  a bijection $h:\S^1 \ra \S^2$ such that:
  \begin{compactenum}
  \item $h(s^1_{0})=s^2_{0}$;
  \item for each $(s^1_1, \Pi, s^1_2) \in
    \varrho^1$, $(h(s^1_1), \Pi, h(s^2_2)) \in
    \varrho^2$; and
  \item for each $(s^2_1, \Pi, s^2_2) \in \varrho^2$,
    $(h^{-1}(s^2_1), \Pi, h^{-1}(s^2_2)) \in
    \varrho^1$.
  \end{compactenum}
  We write $A_1 \bijectf{h} A_2$ to explicitly indicate the bijection $h$ from $A_1$ to $A_2$ that induces their shape equivalence.
%\end{definition}

It is easy to see that bijection $h$ preserves the initial states (condition (1)) and transitions (conditions (2) and (3)), but does not require a correspondence between final states.

\begin{lemma}
  Shape equivalence $\sim$ is indeed an equivalence relation.
\end{lemma}
\begin{proof}
  Reflexivity: the identity function trivially satisfies (1)-(3) above.
%%
  Symmetry: let $A \bijectf{h} A$. Given that $h$ is a
  bijection, then $A \bijectf{h^{-1}} A$.
%%
  Transitivity: Let $A_1 \bijectf{h} A_2$ and $A_2
  \bijectf{g} A_3$. Then $A_1 \bijectf{h\;\circ\;g}
  A_3$, where $h \circ g$ is the composition of $h$ and $g$.
\end{proof}

Hence, $\biject$ induce (equivalence) classes of automata with the same shape. Automata for the basic formulae in Theorem~\ref{thm:rv-ltl} belong to the same class.

\begin{lemma}
  For each \LDLf formula $\varphi$, $A(\varphi)$, $A(\neg \varphi)$,
  $A(\DIAM{\pref_{\varphi}}\Endt)$ and $A(\DIAM{\pref_{\neg
      \varphi}}\Endt)$ are in the same equivalence class by $\biject$.
\end{lemma}
\begin{proof}
  From automata theory, $A(\neg \varphi)$ can be obtained from
  $A(\varphi)$ by switching the final states with the non-final
  ones. Hence, the identity $i: \S^{\varphi} \ra \S^{\varphi}$ is such that $A(\varphi) \bijectf{i} A(\neg \varphi)$.
%%
  Moreover, $A(\varphi) \biject A(\DIAM{\pref_{\varphi}}\Endt) \biject
  A(\DIAM{\pref_{\neg \varphi}}\Endt)$ as $A(\DIAM{\pref_{\varphi}}\Endt)$, respectively, $A(\DIAM{\pref_{\neg \varphi}}\Endt)$, can be obtained from $A(\varphi)$, respectively, $A(\neg \varphi)$, by setting as final states all states from which there exists a non-zero length path to a final state of $A(\varphi)$, respectively, $A(\neg \varphi)$, as explained in the proof of Lemma~\ref{lemma:prefRE}. Hence, again, the identity relation $i$ is such that $A(\varphi) \bijectf{i} A(\DIAM{\pref_{\varphi}}\Endt) \bijectf{i}
  A(\DIAM{\pref_{\neg \varphi}}\Endt)$.
\end{proof}

As the last step for proving that automata for the four formulae in Theorem~\ref{thm:rv-ltl} are in the same class, we show that the formula conjunction does not alter shape equivalence, in the following precise sense.

\begin{theorem}
  Let $\varphi_1$, $\varphi_2$, $\psi_1$ and $\psi_2$ be \LDLf
  formulae  so that $A(\varphi_1) \biject A(\psi_1)$ and
  $A(\varphi_2) \biject A(\psi_2)$. Then $A(\varphi_1 \land
  \varphi_2) \biject A(\psi_1 \land \psi_2)$.
\end{theorem}
\begin{proof}
  From the semantics of \LDLf and Theorem~\ref{thm:automataSoundness}, it
  follows that $A(\varphi_1 \land \varphi_2) \equiv A(\varphi_1) \cap
  A(\varphi_2)$.
  Recall that states of $A(\varphi_1) \cap
  A(\varphi_2)$ are ordered pairs $(s^{\varphi_1}, s^{\varphi_2}) \in
  \S^{\varphi_1} \times \S^{\varphi_2}$.
Let $h_1$ and $h_2$ be bijections such that $A(\varphi_1) \bijectf{h_1} A(\psi_1)$ and
  $A(\varphi_2) \bijectf{h_2} A(\psi_2)$. We use $h_1$ and $h_2$ to construct a new bijection  $h:
  \S^{\varphi_1} \times \S^{\varphi_2} \ra \S^{\psi_1} \times
  \S^{\psi_2}$ such that $h(s^{\varphi_1},
  s^{\varphi_2})=(h_1(s^{\varphi_1}), h_2(s^{\varphi_2}))$. We show that $h$ satisfies criteria (1)-(3) of shape equivalence, hence inducing
 $A(\varphi_1 \land \varphi_2) \bijectf{h} A(\psi_1
  \land \psi_2)$.
%%
  The starting state $s_0^{\varphi_1 \land \varphi_2}$ of $A(\varphi_1 \land \varphi_2)$ corresponds to
    $(s_0^{\varphi_1},
  s_0^{\varphi_2})$ by definition of $A(\varphi_1) \cap
  A(\varphi_2)$. At the same time, $s_0^{\psi_1 \land \psi_2}=(h_1(s_0^{\varphi_1}),
  h_2(s_0^{\varphi_2}))=(s_0^{\varphi_1}, s_0^{\varphi_2})$ by
  definition of $h$, which proves (1).
%%
  Now, consider a transition $((s^{\varphi_1}_1, s^{\varphi_2}_1), \Pi, (s^{\varphi_1}_2,
  s^{\varphi_2}_2))$ in $\varrho^{\varphi_1 \land \varphi_2}$. By construction, this means that there exist transitions $(s^{\varphi_1}_1, \Pi,
  s^{\varphi_1}_2) \in \varrho^{\varphi_1}$ and $(s^{\varphi_2}_1,
  \Pi, s^{\varphi_2}_2) \in \varrho^{\varphi_2}$. Since
  $A(\varphi_1) \bijectf{h_1} A(\psi_1)$ and $A(\varphi_2)
  \bijectf{h_2} A(\psi_2)$, we have that $(h_1(s^{\varphi_1}_1), \Pi,
  h_1(s^{\varphi_1}_2)) \in \varrho^{\psi_1}$ and
  $(h_2(s^{\varphi_2}_1), \Pi, h_2(s^{\varphi_2}_2)) \in
  \varrho^{\psi_2}$. It follows that $((h_1(s^{\varphi_1}_1),
  h_2(s^{\varphi_2}_1)), \Pi, (h_1(s^{\varphi_1}_2),
  h_2(s^{\varphi_2}_2))) \in \varrho^{\psi_1 \land \psi_2}$, which
  proves (2). Condition (3) is proved analogously with $h^{-1}$.
\end{proof}


\begin{corollary}
  Given an \LDLf formula $\varphi$, automata $A(\varphi \land \DIAM{\pref_{\lnot\varphi}}\Endt)$,
  $A(\lnot\varphi \land \DIAM{\pref_{\varphi}}\Endt)$,
  $A(\DIAM{\pref_{\varphi}}\Endt\land \lnot
  \DIAM{\pref_{\lnot\varphi}}\Endt)$ and
  $A(\DIAM{\pref_{\lnot\varphi}}\Endt\land \lnot
  \DIAM{\pref_{\varphi}}\Endt)$ are in the same equivalence class by
  $\biject$.
\end{corollary}

\input{monitoringAutomataColored}

This result tells that the automata of the formulae used to capture the RV states of an \LDLf formula of interest, as captured by Theorem~\ref{thm:rv-ltl}, are identical modulo final states. In addition, by definition of the four \LDLf formulae, we directly get that each state is marked as final by one and only one of such automata. This, in turn, allows us to merge all the four automata together into a single automaton, provided that we recall, for each state in the automaton, which of the four formula marks it as final (which corresponds to declare to which of the four RV states it corresponds). In practice, we can simply build the automaton $A(\varphi)$ for $\varphi$, and ``color'' each state in the automaton according to its corresponding RV state. This can be realized with the following, direct procedure. We first build $A(\varphi) =
  (2^\Prop,\S,s_{0}, \varrho,
  S_{f})$, with $S_{f}$ the set of its final states, and, for each $s \in \S$, we compute the set $Reach(s)$ of states reachable from $s$. Then:
\begin{compactitem}[$\bullet$]
\item if
\begin{inparaenum}[\it (i)]
\item $s \in S_{f}$,
\item $Reach(s) \not \subseteq S_{f}$, and
\item $Reach(s) \cap \set{s_{f}} \not = \emptyset$,
 \end{inparaenum}
 then we mark $s$ as $\temptrue$;
\item if \begin{inparaenum}[\it (i)]
\item $s \not \in S_{f}$,
\item  $Reach(s) \not \subseteq (\S \setminus S_{f})$, and
\item $Reach(s) \cap S_{f} \not = \emptyset$,
 \end{inparaenum}
 then we mark $s$ as $\tempfalse$;
\item if \begin{inparaenum}[\it (i)]
\item $s \in S_{f}$ and
\item $Reach(s) \subseteq S_{f}$,
 \end{inparaenum}
then we mark $s$ as $\permtrue$;
\item if \begin{inparaenum}[\it (i)]
\item $s \not \in S_{f}$ and
\item $Reach(s) \subseteq (\S \setminus S_{f})$,
 \end{inparaenum}
 then we mark $s$ as $\permfalse$.
\end{compactitem}
It is easy to see that the four bullets above match the four ones of Theorem~\ref{thm:rv-ltl}. The soundness of the marking immediately follows from the definitions and results in the previous section.


\begin{example}
Figure~\ref{fig:monitoringAutColored} depicts the colored automaton for the formula in Example~\ref{ex:monitoringAutomata} and Figure~\ref{subfig:general}. States $s_0$ and $s_1$, which were final in the automaton for $\pi \models \rvass{\varphi}{\tempfalse}$, are indeed marked as $\temptrue$ (orange, dashed line); state $s_2$, which was final in the automaton for $\pi \models \rvass{\varphi}{\temptrue}$, is marked as $\temptrue$ (blue, solid thin line); state $s_3$, which was final in the automaton for $\pi \models \rvass{\varphi}{\permtrue}$, is marked with $\permtrue$ (green, solid thick line); and, lastly, state $s_4$, which was final in the automaton for $\pi \models \rvass{\varphi}{\permfalse}$, is marked with $\permfalse$ (red, dotted line).
\end{example}

Upon building the colored automaton, we can determinize it and keep it \emph{untrimmed}, that is, including trap states from which no final state can be reached. In this way, every symbol from the entire supporting set $\Prop$ is accepted by the automaton in each of its states. This becomes then our \emph{monitor}.

We conclude by noticing that the presented solution is very flexible, as the reachability analysis can be performed on-the-fly: indeed, this is the procedure we actually implemented in our runtime verification tool, as explained in Section~\ref{sec:implementation}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> 4-monitoring-ldlf.tex <==
\subsection{Monitoring \LDLf Formulae}
\label{sec:monitor}
As pointed out in the previous section, the core issue in monitoring is
prefix recognition. \LTLf is not expressive enough to talk about
prefixes of its own formulae. Roughly speaking, given an \LTLf formula,
the language of its possibly good prefixes cannot be in
general described as an \LTLf formula. For such a reason, building a
monitor usually requires direct manipulation of the automaton for
the formula.
%%

\LDLf, instead, can capture any nondeterministic automaton as a formula, and it has
 the
capability of expressing properties on prefixes. We
can exploit such an extra expressivity to capture
the monitoring condition in a direct and elegant way.
%%
We start by showing how to construct formulae representing (the
language of) prefixes of other formulae, and then we show how to
use them in the context of monitoring.

Technically, given an \LDLf formula $\varphi$, it is possible to
express the language $\L_{\possgood}(\varphi)$ with an \LDLf formula
$\varphi'$. Such a formula is obtained in two steps.

\begin{lemma}
\label{lemma:prefRE}
  Given an \LDLf formula $\varphi$, there exists a regular expression
  $\pref_{\varphi}$ such that $\L(\pref_{\varphi}) =
  \L_{\possgood}(\varphi)$.
\end{lemma}

\begin{proof}
  The proof is constructive. We build the \NFA $A(\varphi)$ for $\varphi$. We then build a new \NFA $A_{\possgood}(\varphi)$ by taking
  $A(\varphi)$ and setting as final states all states from which we can reach a final state of $A(\varphi)$. The so-obtained \NFA $A_{\possgood}(\varphi)$
  is such that
  $\L(A_{\possgood}(\varphi))=\L_{\possgood}(\varphi)$. Since \NFA
  are exactly as expressive as regular expressions, we can translate
  $A_{\possgood}(\varphi)$ to the corresponding regular expression $\pref_{\varphi}$.
\end{proof}


Since \LDLf is as expressive as regular expressions
(cf.~\cite{DegVa13}), we can translate $\pref_{\varphi}$ into an
equivalent \LDLf formula.

\begin{theorem}
  \label{th:prefFormula}
  Given an \LDLf formula $\varphi$,
  \[\begin{array}{l}
    \pi\in \L_{\possgood}(\varphi)\; \text{iff}\; \pi\models \DIAM{\pref_{\varphi}}\Endt\\
    \pi\in \L_{\necgood}(\varphi)\; \text{iff}\; \pi\models \DIAM{\pref_{\varphi}}\Endt\land \lnot \DIAM{\pref_{\lnot\varphi}}\Endt\\
  \end{array}
  \]
\end{theorem}
\begin{proof}
  Any regular expression $\rho$, and hence any regular language, can be captured in \LDLf as $\DIAM{\rho}\Endt$.
Specifically, the language $\L_{\possgood}(\varphi)$ is captured by $\DIAM{\pref_{\varphi}}\Endt$, and the language $\L_{\necgood}(\varphi)$,
which is equivalent to $\L_{\possgood}(\varphi) \setminus \L_{\possgood}(\neg \varphi)$, is captured by $\DIAM{\pref_{\varphi}}\Endt\land \lnot \DIAM{\pref_{\lnot\varphi}}\Endt$.
\end{proof}
%%
In other words, given an \LDLf formula $\varphi$, formula
$\varphi'=\DIAM{\pref_{\varphi}}\Endt$ is an \LDLf formula such that
$\L(\varphi') = \L_{\possgood}(\varphi)$. Similarly for $\L_{\necgood}(\varphi)$.
%%
% Observe that we can now recognize if a trace $\pi$ belongs to the good
% prefixes of a formula by simply checking whether the previous formula
% is true in $\pi$.

Exploiting this result, and the results in
Proposition \ref{thm:RVLDL}, we reduce the evaluation of RV states to the
standard evaluation of \LDLf formulae over a (partial) trace. Formally:

\begin{theorem}
\label{thm:rv-ltl}
Let $\pi$ be a trace. The following equivalences hold:
  \begin{compactitem}[$\bullet$]
  \item $\pi \models \rvass{\varphi}{\temptrue}$\; iff\; $\pi \models
    \varphi \land \DIAM{\pref_{\lnot\varphi}}\Endt$;
%%
  \item $\pi \models \rvass{\varphi}{\tempfalse}$\; iff\; $\pi \models
    \lnot\varphi \land \DIAM{\pref_{\varphi}}\Endt$;
%
  \item $\pi \models \rvass{\varphi}{\permtrue}$\; iff\;
    $\pi \models \DIAM{\pref_{\varphi}}\Endt\land \lnot
    \DIAM{\pref_{\lnot\varphi}}\Endt$;
%
  \item $\pi \models \rvass{\varphi}{\permfalse}$\; iff\;
    $\pi \models \DIAM{\pref_{\lnot\varphi}}\Endt\land \lnot
    \DIAM{\pref_{\varphi}}\Endt$.
  \end{compactitem}
\end{theorem}
\begin{proof}
  The theorem follows directly from Proposition~\ref{thm:RVLDL} and
  Theorem~\ref{th:prefFormula}.
\end{proof}

\input{monitoringAutomata}

This result provides an actual procedure to return the RV state of an \LDLf formula $\varphi$: we build four automata, one for each of the four formulae above, and then follow the evolution of the trace $\pi$ simultaneously on each one of them. Since Proposition~\ref{prop:lang-partitions} proves that the languages of the four automata are a partition for the set of all languages over $(2^\P)^*$, we are guaranteed that, at each step, one and only one automaton is in a final state, namely, one and only one truth value is returned as output of the monitoring procedure.

\begin{example} \label{ex:monitoringAutomata}
Figure~\ref{subfig:general} shows the graphical representation of the automaton for formula $\Phi :=\Next(a \ra (\Wnext b))$, where $s_0$ is the initial state and final states are double-circled. Moreover, for the sake of readability, labels on edges are logical formulae, a shortcut for every interpretation satisfying that formula, e.g., the edge labeled with $\neg a$ from state $s_1$ to $s_2$ is a shortcut for $(s_1, \set{\neg a, b}, s_2), (s_1, \set{\neg a, \neg b}, s_2) \in \varrho$. Formula $\Phi$ intuitively requires that. in the next step, if $a$ is performed then either the trace ends (for the semantics of the weak next operator $\Wnext$) or, if it continues, then it is forced to continue by performing $b$. Figures~\ref{subfig:temptrue}~--~\ref{subfig:false} represent the four automata for monitoring the different RV truth values. More specifically:
\begin{compactitem}[$\bullet$]
\item The automaton in Figure~\ref{subfig:temptrue} is used to check wether $\pi \models \rvass{\varphi}{\temptrue}$. Indeed, its final state is $s_2$, which corresponds to the subset of the final states in the original automaton from which some non-final state (in this case $s_4$) can still be reached.
\item The automaton in Figure~\ref{subfig:tempfalse} is used to check wether $\pi \models \rvass{\varphi}{\tempfalse}$. Indeed its final states are $s_0$ and $s_1$, which correspond to the subset of the non-final states in the original automaton from which some final state (in this case $s_3$) can still be reached.
\item The automaton in Figure~\ref{subfig:true} is used to check wether $\pi \models \rvass{\varphi}{\permtrue}$. Indeed, its final state is $s_3$, which corresponds to the subset of the final states in the original automaton from which no non-final state can ever be reached.
\item The automaton in Figure~\ref{subfig:false} is used to check wether $\pi \models \rvass{\varphi}{\permfalse}$. Indeed, its final state is $s_4$, which corresponds to the subset of the final states in the original automaton from which no final state can ever be reached.
\end{compactitem}
\end{example}


In the next section, we prove that using four automata is indeed redundant, and that monitoring can be performed by making use of just a single automaton that retains, at once, all the necessary monitoring information.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> 7-implementation-backend.tex <==
\subsection{Reasoning Component}
\label{sec:backend}
The reasoning component of the \textsc{LDL Monitor}, FLLOAT (``From \LTLf/\LDLf To AuTomata'', \url{https://github.com/RiccardoDeMasellis/FLLOAT}) implements the logics of the runtime verification by building the automaton of the reference model \LDLf constraints with the algorithms presented in Section~\ref{sec:automaton}.

\begin{figure}
\includegraphics[scale=1]{sw-component}
\centering
\caption{UML-like diagram of the backend main components.}
\label{fig:conceptual-modules}
\end{figure}

The FFLOAT code has been implemented in the Java language and exploits the inheritance features of object oriented languages. It is made up by several conceptual modules and makes use of external libraries as shown by the UML-like diagram in Figure~\ref{fig:conceptual-modules}, where the main java classes are depicted by the usual rectangles, their surrounding boxes represent the conceptual modules they belong to and dashed arrows show the dependencies. In what follows we will address each conceptual module separately.

\begin{figure} 
\includegraphics[scale=.3]{uml-formula}
\centering
\caption{UML-like diagram of the classes for \LDLf formulae.} 
\label{fig:uml-formula}
\end{figure}

\paragraph{Formulae} It contains classes and methods to represent and manipulate logical formulae. Classes in this module have a complex hierarchy, as formulae are characterized by several independent aspects: the language (\LDLf, \LTLf, \RE); the structure (atomic, unary, binary) and the temporal characterization (local or temporal). Since Java does not allow multiple inheritance, such a hierarchy has been reproduced by a suitable use of subclasses and interfaces. Besides, formulae are implemented with an inductive structure, i.e., formulae have as instance variable a formula if unary, or two if binary, which allows us to elegantly implement all recursive functions for their manipulation.
%%
Each formula implements the interface \texttt{Formula}, which is then extended by six interfaces, each representing a specific characteristic: \texttt{Temporal} if the formula contains a temporal operator; \texttt{Local} if it does not; \texttt{BooleanOp} if its main operator is a boolean operator; \texttt{Atomic} if it is atomic, i.e., if it is (propositional) $true$ (abstract class \texttt{TrueLocal}), (propositional) $false$ (abstract class \texttt{FalseLocal}) or a propositional variable \texttt{LocalVar}; \texttt{Unary} if its main operator is a unary operator and lastly \texttt{Binary} if it is instead binary. Besides, \texttt{BooleanOp} is extended by interfaces representing the usual boolean operators, such as \texttt{Not}, which also extends \texttt{Unary}, and \texttt{And}, which also extends \texttt{Binary}, and so on for the other boolean connectives. We remark that it is necessary to express such different characteristics by means of interfaces, as each formula is indeed a combination of those.
%%
At a lower level of abstraction, we have three main type of formulae: \LDLf, \LTLf and \RE each of which is again an interface extending \texttt{Formula}. Here we provide a detailed description of the structure of \LDLf formulae only, but the same ideas also hold for \LTLf and \RE formulae. Figure~\ref{fig:uml-formula} provides a UML-like class diagram for \LDLf formulae, where dashed boxes represent interfaces, simple boxes are abstract classes; boxes with bold text are classes and arrows mean both extends or implements, depending on whether the extending/implementing entity is an interface or a (abstract) class. \texttt{LDLf} extends \texttt{Formula}, and is extended by interface \texttt{LDLfTemp} (which also extends \texttt{Temporal}); \texttt{LDLfBooleanOp} (which also extends \texttt{BooleanOp}) and \texttt{LDLfLocal} (which also extends \texttt{Local}). Moreover, \texttt{LDLf} is implemented by abstract classes \texttt{LDLfUnary} and \texttt{LDLfBinary}, which also extend \texttt{Unary} and \texttt{Binary}, respectively.
%%
An atomic \LDLf formula is clearly local, and, as presented in Section~\ref{sec:LTLf-LDLf}, can be \texttt{LDLfLocalTrue}, i.e., the propositional $true$ (hence extending \texttt{TrueLocal} and implementing \texttt{LDLfLocal}) or, analogously, \texttt{LDLfLocalFalse} or \texttt{LDLfLocalVar}.
%%
Other local \LDLf formulae are boolean combinations of other local formulae, hence they all implement interface \texttt{LDLfBooleanOpLocal}, such as \texttt{LDLfLocalNot} (which also implements \texttt{Not}) and \texttt{LDLfLocalAnd} (which also implements \texttt{And}). \texttt{LDLfBooleanOpTemp} formulae have an analogous structure.
%%
The other \LDLf temporal formulae are the atomic \texttt{LDLftt} and \texttt{LDLfff} formulae and formulae with a temporal operator, thus extending abstract class \texttt{LDLfTempOpTemp}, that is, \texttt{LDLfBox} and \texttt{LDLfDiamond} formulae.

Although such a hierarchical structure may seem cumbersome, when dealing with a relevant number of classes it is essential to keep the code modular. As an example, let us consider the negation normal form (NNF) of a formula: regardless if a formula is a \texttt{LDLfLocalAnd}, \texttt{LDLfTempAnd}, \texttt{LTLfLocalAnd} or \texttt{LTLfTempAnd}, the logic for transforming an \texttt{And} formula in NNF is the same. Indeed, non-static method \emph{nnf()} has been implemented as a \emph{default} method in the \texttt{And} interface, and it is hence inherited by all implementing classes. Similar considerations also hold for method \emph{getSig()}, which returns the set of propositional variables appearing in the formula, as it can be defined as a \emph{default} method in interfaces \texttt{Unary} and \texttt{Binary}. Another notable example is the \emph{delta()} method, which implements the delta function in Figure~\ref{fig:delta}, which, being the same for all \texttt{LDLfLocal} formulae, has been implemented as a \emph{default} method in interface \texttt{LDLfLocal}. Also, methods returning sub-formulae, such as \emph{getNested}, \emph{getLeft} and \emph{getRight} are defined in the abstract classes \texttt{LDLfUnary} and \texttt{LDLfBinary}.



\paragraph{Automaton construction} The main functionality FLLOAT provides is the automaton generation for an \LTLf/\LDLf formula $\varphi$ given as input, which is implemented in the static method \emph{ldlf2Automaton} of class \texttt{AutomatonUtils}. The whole procedure works as follows. First, the formula is parsed and an \texttt{LTLf} or \texttt{LDLf} object is created. This is achieved by classes that are previously and automatically generated by ANTLR\footnote{\url{http://www.antlr.org}} starting from grammar files. Then, if the input formula is \LDLf, then it is translated in negation normal form (\emph{nnf()} method) and the algorithm for the automata generation is called. Conversely, if it is \LTLf, it must be first converted to \LDLf by method \emph{toLDLf()} implementing the translation explained in Section~\ref{sec:LTLf-LDLf}. Once an \LDLf formula $\varphi$ in negation normal form has been obtained, the automaton is generated with Algorithm~\ref{fig:algo}. The method \emph{ldlf2Automaton} consists of two nested cycles, the outer on states in $\S$ yet to be analyzed and the inner on interpretation for $\Prop$ or the empty trace (line $8$ of Algorithm~\ref{fig:algo}): at each iteration $\delta(s, \Theta)$ is computed, where $s \in \S$ and $\Theta \in 2^\Prop \cup \epsilon$, possibly generating new states $q'$ to be added to the set of states to be analyzed along with the respective transitions (line $8-9$ of Algorithm~\ref{fig:algo}). Since function $\delta$ is recursively defined on the structure of \LDLf formulae, it is implemented by the recursive non-static \emph{delta} method of \texttt{LDLf} class, exploiting the java inheritance features. The Tweety library\footnote{\url{http://tweetyproject.org}} is used to compute the models, i.e., $q'$ states, of the formula $\bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Theta)$ in line $8$ of Algorithm~\ref{fig:algo}.
%%
The procedure starts by analyzing $\atomize{\varphi}$, the only state in $\S$, and ends when all states have been analyzed and no others have been generated in the meanwhile.
%%
The data structures for automata are defined in the jautomata library\footnote{\url{https://github.com/abailly/jautomata}}, which also provides methods for automata manipulation, such as union, intersection, trimming and determinization.


\paragraph{Runtime Verification} The runtime verification functionalities are provided by the \texttt{ExecutableAutomaton} class. An executable automaton is essentially a deterministic automaton (every \NFA can be determinized) with a reference to the current state. When an executable automaton is created from an automaton, the current state is set to the initial state (by construction there is always a unique initial state). The idea is to navigate the automaton and return \RV truth values while events are executed. Recalling the results presented in Section~\ref{sec:colored-proof}, each automaton state represents a \RV truth value. Hence, an operative way to implement a \RV monitor is to analyze one-by-one the occurring events and to perform the corresponding transitions on the automaton of the constraints. Each time a state change is triggered by a transition leading to state $s$, we calculate $Reach(s)$ and return the corresponding truth value.
%%
In our implementation when a new event is executed, the non-static method $step$, taking $\Theta \in 2^\Prop \cup \set{\varepsilon}$ as input, is called, updating the current state by traversing the corresponding $\Theta$ transition. Method $currentRVTruthValue$ computes $Reach$ for the current state and returns one among $\permtrue, \permfalse, \temptrue, \tempfalse$ as explained at the end of Section~\ref{sec:colored-proof}, thus effectively implementing the \RV semantics.


















\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End: 

==> monitoringAutomata.tex <==

%%% First automaton, top-left
\begin{figure}[h!] \label{fig:monitoringAutomata}
  \centering
\begin{subfigure}[b]{1\textwidth}
\centering
\begin{tikzpicture} [->,>=latex,auto,node distance=1cm, very thick]

\node[state] (s1) {$s_1$};

\node[istate] (s0) [above left=1cm of s1, anchor=south] {$s_0$};

\node[state, accepting] (s2) [above right=1 cm of s1, anchor=south] {$s_2$};

\node[state, accepting] (s3) [right=1 cm of s1, anchor=west] {$s_3$};

\node[state] (s4) [right=1cm of s2, anchor=west] {$s_4$};

\path
(s0) edge node [pos=0.2, below left, align=center] {$true$} (s1)

(s1) edge node [pos=0.5] {$a$} (s2)
      edge node [above] {$\neg a$} (s3)

(s2) edge node [above] {$\neg b$} (s4)
      edge node [pos=0.5] {$b$} (s3)

(s3) edge [loop below] node {$true$} (s3)

(s4) edge [loop below] node [below, align=center] {$true$} (s4);
\end{tikzpicture}
\caption{Graphical representation of the automaton for $\Phi:=\Next (a \ra (\Wnext b))$.}
\label{subfig:general}
\end{subfigure}

\begin{subfigure}[b]{0.4\textwidth} \centering
\begin{tikzpicture} [->,>=latex,auto,node distance=1cm, very thick]

\node[state] (s1) {$s_1$};

\node[istate] (s0) [above left=1cm of s1, anchor=south] {$s_0$};

\node[state, accepting] (s2) [above right=1 cm of s1, anchor=south] {$s_2$};

\node[state] (s3) [right=1 cm of s1, anchor=west] {$s_3$};

\node[state] (s4) [right=1cm of s2, anchor=west] {$s_4$};

\path
(s0) edge node [pos=0.2, below left, align=center] {$true$} (s1)

(s1) edge node [pos=0.5] {$a$} (s2)
      edge node [above] {$\neg a$} (s3)

(s2) edge node [above] {$\neg b$} (s4)
      edge node [pos=0.5] {$b$} (s3)

(s3) edge [loop below] node {$true$} (s3)

(s4) edge [loop below] node [below, align=center] {$true$} (s4);
\end{tikzpicture}
\caption{Graphical representation of the automaton for $\Phi \land \DIAM{\pref_{\lnot\Phi}}\Endt$, used to check uf $\pi \models \rvass{\varphi}{\temptrue}$.}
\label{subfig:temptrue}
\end{subfigure} \qquad \begin{subfigure}[b]{0.4\textwidth} \centering
\begin{tikzpicture} [->,>=latex,auto,node distance=1cm, very thick]

\node[state, accepting] (s1) {$s_1$};

\node[istate, accepting] (s0) [above left=1cm of s1, anchor=south] {$s_0$};

\node[state] (s2) [above right=1 cm of s1, anchor=south] {$s_2$};

\node[state] (s3) [right=1 cm of s1, anchor=west] {$s_3$};

\node[state] (s4) [right=1cm of s2, anchor=west] {$s_4$};

\path
(s0) edge node [pos=0.2, below left, align=center] {$true$} (s1)

(s1) edge node [pos=0.5] {$a$} (s2)
      edge node [above] {$\neg a$} (s3)

(s2) edge node [above] {$\neg b$} (s4)
      edge node [pos=0.5] {$b$} (s3)

(s3) edge [loop below] node {$true$} (s3)

(s4) edge [loop below] node [below, align=center] {$true$} (s4);
\end{tikzpicture}
\caption{Graphical representation of the automaton for $\neg \Phi \land \DIAM{\pref_{\Phi}}\Endt$, used to check if $\pi \models \rvass{\varphi}{\tempfalse}$.}
\label{subfig:tempfalse}
\end{subfigure}

\vspace{0.2cm}

\begin{subfigure}[b]{0.4\textwidth} \centering
\begin{tikzpicture} [->,>=latex,auto,node distance=1cm, very thick]

\node[state] (s1) {$s_1$};

\node[istate] (s0) [above left=1cm of s1, anchor=south] {$s_0$};

\node[state] (s2) [above right=1 cm of s1, anchor=south] {$s_2$};

\node[state, accepting] (s3) [right=1 cm of s1, anchor=west] {$s_3$};

\node[state] (s4) [right=1cm of s2, anchor=west] {$s_4$};

\path
(s0) edge node [pos=0.2, below left, align=center] {$true$} (s1)

(s1) edge node [pos=0.5] {$a$} (s2)
      edge node [above] {$\neg a$} (s3)

(s2) edge node [above] {$\neg b$} (s4)
      edge node [pos=0.5] {$b$} (s3)

(s3) edge [loop below] node {$true$} (s3)

(s4) edge [loop below] node [below, align=center] {$true$} (s4);
\end{tikzpicture}
\caption{Graphical representation of the automaton for $\DIAM{\pref_{\Phi}}\Endt \land \neg \DIAM{\pref_{\neg \Phi}}\Endt$, used to check if $\pi \models \rvass{\varphi}{\permtrue}$.}
\label{subfig:true}
\end{subfigure} \qquad \begin{subfigure}[b]{0.4\textwidth} \centering
\begin{tikzpicture} [->,>=latex,auto,node distance=1cm, very thick]

\node[state] (s1) {$s_1$};

\node[istate] (s0) [above left=1cm of s1, anchor=south] {$s_0$};

\node[state] (s2) [above right=1 cm of s1, anchor=south] {$s_2$};

\node[state] (s3) [right=1 cm of s1, anchor=west] {$s_3$};

\node[state, accepting] (s4) [right=1cm of s2, anchor=west] {$s_4$};

\path
(s0) edge node [pos=0.2, below left, align=center] {$true$} (s1)

(s1) edge node [pos=0.5] {$a$} (s2)
      edge node [above] {$\neg a$} (s3)

(s2) edge node [above] {$\neg b$} (s4)
      edge node [pos=0.5] {$b$} (s3)

(s3) edge [loop below] node {$true$} (s3)

(s4) edge [loop below] node [below, align=center] {$true$} (s4);
\end{tikzpicture}
\caption{Graphical representation of the automaton for $\DIAM{\pref_{\neg \Phi}}\Endt \land \neg \DIAM{\pref_{\Phi}}\Endt$, used to check if $\pi \models \rvass{\varphi}{\permfalse}$.}
\label{subfig:false}
\end{subfigure}
\caption{Automata used to monitor the four RV truth values of formula $\Next(a \ra (\Wnext b))$.}
\end{figure}


\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% save-place: t
%%% End:





\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% save-place: t
%%% End:
